The TROY project: Searching for co-orbital bodies to known planets. I. Project goals and first results from archival radial velocity

The detection of Earth-like planets, exocomets or Kuiper belts show that the different components found in the solar system should also be present in other planetary systems. Trojans are one of these components and can be considered fossils of the first stages in the life of planetary systems. Their detection in extrasolar systems would open a new scientific window to investigate formation and migration processes. In this context, the main goal of the TROY project is to detect exotrojans for the first time and to measure their occurrence rate (eta-Trojan). In this first paper, we describe the goals and methodology of the project. Additionally, we used archival radial velocity data of 46 planetary systems to place upper limits on the mass of possible trojans and investigate the presence of co-orbital planets down to several tens of Earth masses. We used archival radial velocity data of 46 close-in (P<5 days) transiting planets (without detected companions) with information from high-precision radial velocity instruments. We took advantage of the time of mid-transit and secondary eclipses (when available) to constrain the possible presence of additional objects co-orbiting the star along with the planet. This, together with a good phase coverage, breaks the degeneracy between a trojan planet signature and signals coming from additional planets or underestimated eccentricity. We identify nine systems for which the archival data provide 1-sigma evidence for a mass imbalance between L4 and L5. Two of these systems provide 2-sigma detection, but no significant detection is found among our sample. We also report upper limits to the masses at L4/L5 in all studied systems and discuss the results in the context of previous findings.

==> Table_Decision.tex <==
\begin{table}[]
\setlength{\extrarowheight}{3pt}
\small
\caption{Definition of the qualitative description of the results for the analyzed systems. See also Table~\ref{tab:maxmass}.}
\begin{center}
\begin{tabular}{l|lll}
\hline
\hline
   Odd ratio     & \multicolumn{3}{c}{Posterior shape} \\
$(\ln{O_{t,nt}})$ & Gaussian  &  Truncated  &  Exponential \\ \hline
$<-1.1$          & Inconclusive            & Upper limit          & Upper limit \\
$\in [-1.1,0]$   & Weak cand.           & Upper limit          & Upper limit \\
$\in [0,1.1]$    & Candidate            & Weak cand.           & -           \\
$\in [1.1,2.3]$  & Strong cand.         & Candidate            & -           \\
$\in [2.3,4.6]$  & Tentative det.  & Strong cand.         & -           \\
$>4.6$           & Positive det.   & Tentative det.       & -           \\

\hline
\hline
\end{tabular}
\end{center}
\label{tab:decision}
\end{table}%



==> Table_Odds.tex <==
\begin{table*}[]
\setlength{\extrarowheight}{5pt}
\caption{Natural logarithm of the Odd values ($\ln{Odd}=\ln{E_{\mathcal{M}_i}}-\ln{E_{\mathcal{M},{\rm best}}}$) for each model with repespect to the model with maximum evidence ($\ln{Odd} = 0$, in bold face).}
\scriptsize
\begin{center}
\begin{tabular}{l|ccc|ccc|ccc}
\hline
\hline
  & \multicolumn{9}{c}{Bayes' factors}   \\ \hline
System  & \multicolumn{3}{c|}{No trojan} & \multicolumn{3}{c|}{Trojan at L$_4$} & \multicolumn{3}{c}{Trojan at L$_5$}  \\

     & {$\mathcal{M}_{1,a}$} & {$\mathcal{M}_{1,b}$} & {$\mathcal{M}_{1,c}$} & {$\mathcal{M}_{2,a}$} & {$\mathcal{M}_{2,b}$} & {$\mathcal{M}_{2,c}$} & {$\mathcal{M}_{3,a}$} & {$\mathcal{M}_{3,b}$} & {$\mathcal{M}_{3,c}$}   \\
\hline


corot-15b            & 	\textbf{0} & 	$-8.09^{+0.74}_{-0.42}$ & 	$-8.12^{+0.76}_{-0.50}$ & 	$-2.18^{+0.61}_{-0.52}$ & 	$-10.72^{+0.52}_{-0.49}$ & 	$-13.21^{+1.0}_{-0.52}$ & 	$-7.25^{+0.70}_{-0.50}$ & 	$-10.07^{+0.73}_{-0.43}$ & 	$-13.26^{+1.0}_{-0.72}$ \\
corot-18b            & 	\textbf{0} & 	$-9.4^{+1.1}_{-1.2}$ & 	$-7.0^{+1.3}_{-1.2}$ & 	$-3.7^{+1.2}_{-1.0}$ & 	$-15.9^{+1.0}_{-1.1}$ & 	$-15.8^{+1.1}_{-1.2}$ & 	$-5.4^{+1.1}_{-1.1}$ & 	$-12.69^{+1.0}_{-0.99}$ & 	$-14.26^{+0.89}_{-1.0}$ \\
corot-1b             & 	\textbf{0} & 	$-7.97^{+0.84}_{-0.60}$ & 	$-25.95^{+1.1}_{-0.77}$ & 	$-3.82^{+0.65}_{-0.56}$ & 	$-14.54^{+0.88}_{-0.74}$ & 	$-24.10^{+1.0}_{-0.83}$ & 	$-5.34^{+1.1}_{-0.62}$ & 	$-13.7^{+1.1}_{-1.1}$ & 	$-21.3^{+1.5}_{-1.2}$ \\
corot-2b             & 	\textbf{0} & 	$-9.8^{+1.9}_{-1.9}$ & 	$-5.86^{+1.3}_{-0.96}$ & 	$-4.8^{+1.3}_{-1.3}$ & 	$-8.8^{+1.5}_{-1.2}$ & 	$-5.6^{+1.6}_{-1.5}$ & 	$-11.0^{+2.1}_{-1.6}$ & 	$-12.7^{+1.8}_{-1.3}$ & 	$-10.7^{+1.6}_{-1.2}$ \\
epic211089792b       & 	$-8.7^{+1.8}_{-1.4}$ & 	$-11.3^{+2.3}_{-2.1}$ & 	$-24.8^{+2.0}_{-1.6}$ & 	\textbf{0} & 	$-10.6^{+1.8}_{-1.5}$ & 	$-8.4^{+2.3}_{-1.7}$ & 	$-15.2^{+2.0}_{-1.9}$ & 	$-30.6^{+2.0}_{-1.5}$ & 	$-37.8^{+1.8}_{-1.2}$ \\
gj3470b              & 	\textbf{0} & 	$-8.08^{+0.50}_{-0.37}$ & 	$-6.92^{+0.55}_{-0.43}$ & 	$-0.78^{+0.42}_{-0.35}$ & 	$-8.82^{+0.73}_{-0.59}$ & 	$-15.68^{+0.74}_{-0.49}$ & 	$-6.33^{+0.45}_{-0.35}$ & 	$-18.53^{+0.62}_{-0.42}$ & 	$-20.25^{+0.82}_{-0.53}$ \\
hat-p-12b            & 	\textbf{0} & 	$-4.90^{+0.43}_{-0.32}$ & 	$-3.84^{+0.39}_{-0.29}$ & 	$-5.88^{+0.41}_{-0.27}$ & 	$-6.67^{+0.67}_{-0.46}$ & 	$-6.36^{+0.79}_{-0.49}$ & 	$-4.64^{+0.35}_{-0.30}$ & 	$-12.82^{+0.76}_{-0.58}$ & 	$-11.98^{+0.63}_{-0.34}$ \\
hat-p-20b            & 	$-332.83^{+0.98}_{-0.50}$ & 	$-27.72^{+1.0}_{-0.64}$ & 	$-11.19^{+1.1}_{-0.61}$ & 	$-339.53^{+1.1}_{-0.54}$ & 	$-29.97^{+1.0}_{-0.64}$ & 	\textbf{0} & 	$-322.58^{+1.0}_{-0.63}$ & 	$-33.99^{+1.1}_{-0.70}$ & 	$-17.28^{+1.1}_{-0.71}$ \\
hat-p-23b            & 	$-4.23^{+0.82}_{-0.60}$ & 	\textbf{0} & 	$-10.42^{+1.0}_{-0.73}$ & 	$-2.37^{+0.81}_{-0.76}$ & 	$-4.85^{+1.1}_{-0.78}$ & 	$-3.78^{+1.1}_{-0.86}$ & 	$-8.33^{+0.79}_{-0.76}$ & 	$-5.72^{+1.1}_{-0.87}$ & 	$-11.33^{+1.2}_{-0.68}$ \\
hat-p-36b            & 	$-1.43^{+0.97}_{-0.93}$ & 	$-0.90^{+1.2}_{-0.97}$ & 	\textbf{0} & 	$-5.61^{+1.0}_{-0.92}$ & 	$-5.4^{+1.4}_{-1.1}$ & 	$-9.20^{+1.4}_{-0.99}$ & 	$-1.83^{+1.0}_{-0.89}$ & 	$-6.0^{+1.6}_{-1.2}$ & 	$-537.73^{+0.83}_{-0.85}$ \\
hat-p-54b            & 	\textbf{0} & 	$-6.36^{+0.71}_{-0.51}$ & 	$-9.45^{+0.60}_{-0.49}$ & 	$-4.45^{+0.54}_{-0.44}$ & 	$-9.69^{+0.96}_{-0.69}$ & 	$-9.32^{+1.1}_{-0.85}$ & 	$-5.36^{+0.47}_{-0.34}$ & 	$-17.77^{+0.68}_{-0.46}$ & 	$-17.44^{+0.93}_{-0.66}$ \\
hats-2b              & 	\textbf{0} & 	$-7.37^{+0.77}_{-0.55}$ & 	$-6.35^{+0.78}_{-0.62}$ & 	$-9.82^{+0.90}_{-0.56}$ & 	$-9.23^{+0.90}_{-0.77}$ & 	$-9.97^{+0.75}_{-0.70}$ & 	$-2.78^{+0.69}_{-0.53}$ & 	$-26.72^{+0.69}_{-0.68}$ & 	$-11.00^{+1.3}_{-0.65}$ \\
hats-9b              & 	\textbf{0} & 	$-7.1^{+1.6}_{-1.1}$ & 	$-11.5^{+1.4}_{-1.3}$ & 	$-3.7^{+1.0}_{-1.0}$ & 	$-10.7^{+1.2}_{-1.3}$ & 	$-10.9^{+1.5}_{-1.3}$ & 	$-4.1^{+1.1}_{-1.1}$ & 	$-25.4^{+1.2}_{-1.0}$ & 	$-14.5^{+1.5}_{-1.4}$ \\
k2-30b               & 	\textbf{0} & 	$-9.88^{+1.0}_{-0.83}$ & 	$-13.44^{+1.2}_{-0.77}$ & 	$-2.8^{+1.1}_{-1.1}$ & 	$-8.25^{+1.2}_{-0.89}$ & 	$-18.61^{+1.1}_{-0.95}$ & 	$-5.4^{+1.3}_{-1.2}$ & 	$-14.76^{+1.3}_{-0.87}$ & 	$-20.8^{+1.4}_{-1.0}$ \\
kepler-17b           & 	\textbf{0} & 	$-6.27^{+0.54}_{-0.39}$ & 	$-10.25^{+0.58}_{-0.44}$ & 	$-4.76^{+0.56}_{-0.51}$ & 	$-10.75^{+0.62}_{-0.48}$ & 	$-14.09^{+0.87}_{-0.46}$ & 	$-3.12^{+0.51}_{-0.38}$ & 	$-12.15^{+0.80}_{-0.53}$ & 	$-14.91^{+0.63}_{-0.51}$ \\
ogle-tr-113b         & 	\textbf{0} & 	$-8.38^{+0.41}_{-0.35}$ & 	$-6.18^{+0.47}_{-0.35}$ & 	$-3.43^{+0.35}_{-0.35}$ & 	$-15.02^{+0.63}_{-0.41}$ & 	$-18.45^{+0.88}_{-0.72}$ & 	$-4.17^{+0.30}_{-0.34}$ & 	$-14.85^{+0.49}_{-0.43}$ & 	$-8.10^{+0.58}_{-0.45}$ \\
ogle-tr-56b          & 	\textbf{0} & 	$-4.13^{+0.46}_{-0.31}$ & 	$-7.01^{+0.46}_{-0.41}$ & 	$-0.75^{+0.47}_{-0.33}$ & 	$-10.12^{+0.62}_{-0.44}$ & 	$-6.76^{+0.54}_{-0.49}$ & 	$-2.41^{+0.50}_{-0.30}$ & 	$-10.57^{+0.54}_{-0.35}$ & 	$-15.03^{+0.57}_{-0.43}$ \\
qatar-1b             & 	\textbf{0} & 	$-7.20^{+0.42}_{-0.53}$ & 	$-6.42^{+0.58}_{-0.39}$ & 	$-0.22^{+0.41}_{-0.38}$ & 	$-8.30^{+0.74}_{-0.78}$ & 	$-9.33^{+0.70}_{-0.59}$ & 	$-7.21^{+0.58}_{-0.39}$ & 	$-16.39^{+0.77}_{-0.61}$ & 	$-11.83^{+0.56}_{-0.44}$ \\
qatar-2b             & 	$-6.83^{+0.60}_{-0.53}$ & 	$-3.65^{+0.65}_{-0.56}$ & 	$-3.91^{+0.62}_{-0.56}$ & 	$-11.67^{+0.64}_{-0.55}$ & 	$-3.40^{+0.73}_{-0.62}$ & 	\textbf{0} & 	$-9.86^{+0.78}_{-0.55}$ & 	$-11.35^{+0.80}_{-0.63}$ & 	$-10.82^{+0.86}_{-0.62}$ \\
tres-3b              & 	$-41.03^{+0.87}_{-0.55}$ & 	$-32.41^{+0.99}_{-0.73}$ & 	$-46.28^{+0.99}_{-0.73}$ & 	$-22.99^{+0.99}_{-0.60}$ & 	$-8.64^{+1.3}_{-0.89}$ & 	\textbf{0} & 	$-47.20^{+1.1}_{-0.84}$ & 	$-42.29^{+1.2}_{-0.83}$ & 	$-37.88^{+1.0}_{-0.74}$ \\
tres-5b              & 	\textbf{0} & 	$-10.18^{+0.43}_{-0.35}$ & 	$-11.93^{+0.80}_{-0.64}$ & 	$-3.93^{+0.52}_{-0.35}$ & 	$-12.67^{+0.71}_{-0.77}$ & 	$-11.09^{+0.78}_{-0.48}$ & 	$-4.94^{+0.50}_{-0.41}$ & 	$-17.18^{+0.75}_{-0.43}$ & 	$-11.08^{+1.1}_{-0.70}$ \\
wasp-103b            & 	\textbf{0} & 	$-9.13^{+0.80}_{-0.61}$ & 	$-8.43^{+0.61}_{-0.49}$ & 	$-3.41^{+0.57}_{-0.46}$ & 	$-10.17^{+0.83}_{-0.84}$ & 	$-17.69^{+0.76}_{-0.53}$ & 	$-3.26^{+0.54}_{-0.44}$ & 	$-12.79^{+0.83}_{-0.74}$ & 	$-39.18^{+0.85}_{-0.80}$ \\
wasp-104b            & 	\textbf{0} & 	$-11.71^{+0.71}_{-0.47}$ & 	$-10.52^{+0.59}_{-0.43}$ & 	$-5.46^{+0.72}_{-0.40}$ & 	$-12.25^{+0.91}_{-0.59}$ & 	$-21.78^{+0.75}_{-0.74}$ & 	$-4.53^{+0.83}_{-0.50}$ & 	$-20.82^{+1.2}_{-0.58}$ & 	$-23.67^{+0.86}_{-0.61}$ \\
wasp-12b             & 	$-204.97^{+0.88}_{-0.81}$ & 	$-36.37^{+1.1}_{-0.96}$ & 	$-36.01^{+0.99}_{-0.88}$ & 	$-212.62^{+0.96}_{-0.81}$ & 	$-45.52^{+1.1}_{-0.96}$ & 	$-43.82^{+1.1}_{-0.88}$ & 	$-86.61^{+1.1}_{-0.92}$ & 	\textbf{0} & 	$-2.28^{+1.2}_{-0.98}$ \\
wasp-135b            & 	\textbf{0} & 	$-1.37^{+0.49}_{-0.38}$ & 	$-0.37^{+0.53}_{-0.36}$ & 	$-0.86^{+0.41}_{-0.33}$ & 	$-5.86^{+0.55}_{-0.51}$ & 	$-2.70^{+0.49}_{-0.53}$ & 	$-2.48^{+0.37}_{-0.36}$ & 	$-6.76^{+0.72}_{-0.56}$ & 	$-2.68^{+0.63}_{-0.48}$ \\
wasp-13b             & 	\textbf{0} & 	$-7.68^{+0.54}_{-0.32}$ & 	$-5.35^{+0.65}_{-0.39}$ & 	$-6.30^{+0.38}_{-0.29}$ & 	$-13.23^{+0.63}_{-0.49}$ & 	$-10.93^{+0.96}_{-0.56}$ & 	$-1.77^{+0.40}_{-0.35}$ & 	$-9.14^{+0.70}_{-0.47}$ & 	$-8.12^{+0.68}_{-0.42}$ \\
wasp-18b             & 	$-136.6^{+1.5}_{-1.0}$ & 	$-4.0^{+1.9}_{-1.1}$ & 	\textbf{0} & 	$-137.5^{+2.2}_{-1.6}$ & 	$-5.6^{+1.7}_{-1.6}$ & 	$-1.7^{+2.1}_{-1.7}$ & 	$-142.4^{+1.7}_{-1.3}$ & 	$-7.9^{+1.8}_{-1.2}$ & 	$-2.0^{+2.0}_{-1.4}$ \\
wasp-19b             & 	\textbf{0} & 	$-2.27^{+0.49}_{-0.51}$ & 	$-3.93^{+0.42}_{-0.55}$ & 	$-5.53^{+0.50}_{-0.30}$ & 	$-8.46^{+0.64}_{-0.44}$ & 	$-11.51^{+0.52}_{-0.51}$ & 	$-2.85^{+0.49}_{-0.42}$ & 	$-4.17^{+0.87}_{-0.77}$ & 	$-8.35^{+0.85}_{-0.78}$ \\
wasp-23b             & 	\textbf{0} & 	$-5.02^{+0.80}_{-0.67}$ & 	$-7.67^{+0.77}_{-0.48}$ & 	$-4.16^{+0.67}_{-0.57}$ & 	$-8.92^{+0.62}_{-0.51}$ & 	$-10.53^{+0.65}_{-0.65}$ & 	$-7.41^{+0.64}_{-0.45}$ & 	$-11.61^{+0.57}_{-0.47}$ & 	$-30.70^{+0.77}_{-0.69}$ \\
wasp-2b              & 	\textbf{0} & 	$-6.6^{+1.8}_{-1.1}$ & 	$-7.7^{+1.6}_{-1.0}$ & 	$-4.29^{+1.4}_{-0.92}$ & 	$-10.4^{+1.6}_{-1.1}$ & 	$-11.2^{+1.5}_{-1.2}$ & 	$-4.6^{+1.5}_{-1.1}$ & 	$-12.5^{+1.8}_{-1.1}$ & 	$-19.1^{+1.9}_{-1.0}$ \\
wasp-35b             & 	\textbf{0} & 	$-8.15^{+0.61}_{-0.42}$ & 	$-7.74^{+0.83}_{-0.57}$ & 	$-2.75^{+0.53}_{-0.37}$ & 	$-10.86^{+0.87}_{-0.62}$ & 	$-12.57^{+0.72}_{-0.81}$ & 	$-0.97^{+0.68}_{-0.43}$ & 	$-13.55^{+0.87}_{-0.46}$ & 	$-9.89^{+0.68}_{-0.64}$ \\
wasp-36b             & 	\textbf{0} & 	$-7.24^{+0.36}_{-0.37}$ & 	$-8.29^{+0.56}_{-0.44}$ & 	$-3.32^{+0.41}_{-0.32}$ & 	$-15.53^{+0.59}_{-0.63}$ & 	$-14.32^{+0.61}_{-0.55}$ & 	$-1.52^{+0.38}_{-0.31}$ & 	$-12.76^{+0.63}_{-0.57}$ & 	$-11.28^{+0.88}_{-0.49}$ \\
wasp-42b             & 	$-13.26^{+0.87}_{-0.58}$ & 	\textbf{0} & 	$-3.00^{+1.0}_{-0.78}$ & 	$-3.92^{+1.1}_{-0.66}$ & 	$-6.85^{+1.2}_{-0.69}$ & 	$-8.14^{+1.1}_{-0.59}$ & 	$-19.36^{+1.2}_{-0.67}$ & 	$-3.99^{+1.1}_{-0.64}$ & 	$-6.32^{+1.1}_{-0.71}$ \\
wasp-43b             & 	\textbf{0} & 	$-8.87^{+0.40}_{-0.34}$ & 	$-7.66^{+0.50}_{-0.37}$ & 	$-3.04^{+0.34}_{-0.24}$ & 	$-12.49^{+0.37}_{-0.49}$ & 	$-8.28^{+0.62}_{-0.58}$ & 	$-2.45^{+0.33}_{-0.28}$ & 	$-10.66^{+0.55}_{-0.48}$ & 	$-14.18^{+0.54}_{-0.52}$ \\
wasp-46b             & 	\textbf{0} & 	$-4.75^{+0.62}_{-0.40}$ & 	$-7.00^{+0.56}_{-0.48}$ & 	$-3.36^{+0.51}_{-0.36}$ & 	$-12.95^{+0.58}_{-0.32}$ & 	$-9.30^{+0.61}_{-0.43}$ & 	$-2.98^{+0.41}_{-0.29}$ & 	$-12.86^{+0.52}_{-0.38}$ & 	$-9.00^{+0.51}_{-0.45}$ \\
wasp-49b             & 	\textbf{0} & 	$-10.52^{+0.44}_{-0.44}$ & 	$-9.24^{+0.43}_{-0.30}$ & 	$-3.75^{+0.32}_{-0.29}$ & 	$-10.79^{+0.43}_{-0.38}$ & 	$-12.91^{+0.63}_{-0.49}$ & 	$-6.21^{+0.40}_{-0.33}$ & 	$-17.68^{+0.68}_{-0.48}$ & 	$-19.71^{+0.71}_{-0.45}$ \\
wasp-4b              & 	$-2.0^{+1.5}_{-1.2}$ & 	$-6.3^{+1.0}_{-1.1}$ & 	$-33.60^{+1.2}_{-0.99}$ & 	\textbf{0} & 	$-7.6^{+1.6}_{-1.4}$ & 	$-12.81^{+0.99}_{-0.95}$ & 	$-11.8^{+1.2}_{-1.0}$ & 	$-7.6^{+1.8}_{-1.5}$ & 	$-7.6^{+1.3}_{-1.4}$ \\
wasp-50b             & 	\textbf{0} & 	$-5.19^{+0.49}_{-0.42}$ & 	$-6.38^{+0.37}_{-0.44}$ & 	$-5.65^{+0.28}_{-0.28}$ & 	$-13.23^{+0.79}_{-0.50}$ & 	$-14.79^{+0.57}_{-0.45}$ & 	$-2.84^{+0.29}_{-0.32}$ & 	$-9.90^{+0.53}_{-0.45}$ & 	$-10.91^{+0.75}_{-0.54}$ \\
wasp-52b             & 	\textbf{0} & 	$-7.16^{+0.92}_{-0.60}$ & 	$-9.88^{+0.93}_{-0.65}$ & 	$-7.52^{+1.2}_{-0.71}$ & 	$-13.05^{+1.3}_{-0.71}$ & 	$-13.50^{+0.99}_{-0.62}$ & 	$-5.72^{+1.2}_{-0.74}$ & 	$-20.62^{+1.1}_{-0.72}$ & 	$-19.95^{+1.2}_{-0.71}$ \\
wasp-5b              & 	$-9.7^{+1.3}_{-1.2}$ & 	$-18.8^{+1.4}_{-1.1}$ & 	$-15.3^{+1.4}_{-1.3}$ & 	$-3.6^{+1.4}_{-1.2}$ & 	$-5.7^{+1.6}_{-1.4}$ & 	\textbf{0} & 	$-14.1^{+1.3}_{-1.3}$ & 	$-22.1^{+1.6}_{-1.3}$ & 	$-31.2^{+1.4}_{-1.2}$ \\
wasp-65b             & 	\textbf{0} & 	$-12.30^{+0.55}_{-0.41}$ & 	$-10.76^{+0.53}_{-0.36}$ & 	$-4.51^{+0.36}_{-0.33}$ & 	$-13.35^{+1.0}_{-0.61}$ & 	$-12.27^{+0.73}_{-0.42}$ & 	$-5.61^{+0.50}_{-0.27}$ & 	$-22.57^{+0.97}_{-0.70}$ & 	$-15.64^{+0.61}_{-0.31}$ \\
wasp-68b             & 	$-5.35^{+0.35}_{-0.25}$ & 	$-7.69^{+0.43}_{-0.38}$ & 	$-5.97^{+0.50}_{-0.31}$ & 	$-11.27^{+0.45}_{-0.30}$ & 	$-15.31^{+0.49}_{-0.45}$ & 	$-15.08^{+0.71}_{-0.49}$ & 	\textbf{0} & 	$-11.96^{+0.85}_{-0.75}$ & 	$-12.23^{+0.68}_{-0.45}$ \\
wasp-77ab            & 	\textbf{0} & 	$-5353.10^{+1.3}_{-0.81}$ & 	$-6.24^{+0.67}_{-0.60}$ & 	$-3.72^{+0.81}_{-0.53}$ & 	$-18.73^{+0.95}_{-0.52}$ & 	$-13.54^{+1.0}_{-0.66}$ & 	$-7.87^{+0.67}_{-0.49}$ & 	$-10.27^{+1.2}_{-0.89}$ & 	$-11.10^{+0.94}_{-0.93}$ \\
wasp-80b             & 	\textbf{0} & 	$-7.19^{+0.72}_{-0.59}$ & 	$-6.66^{+0.76}_{-0.55}$ & 	$-5.16^{+0.47}_{-0.42}$ & 	$-12.70^{+0.95}_{-0.52}$ & 	$-17.54^{+0.70}_{-0.57}$ & 	$-4.38^{+0.42}_{-0.42}$ & 	$-14.32^{+1.1}_{-0.65}$ & 	$-17.10^{+1.2}_{-0.54}$ \\
wasp-98b             & 	\textbf{0} & 	$-10.83^{+0.61}_{-0.46}$ & 	$-6.28^{+0.42}_{-0.39}$ & 	$-3.04^{+0.36}_{-0.29}$ & 	$-24.09^{+0.74}_{-0.48}$ & 	$-13.74^{+0.67}_{-0.45}$ & 	$-4.43^{+0.46}_{-0.31}$ & 	$-18.58^{+0.80}_{-0.58}$ & 	$-12.80^{+0.55}_{-0.33}$ \\
wts-2b               & 	$-0.16^{+0.79}_{-0.59}$ & 	$-10.55^{+0.82}_{-0.60}$ & 	$-7.42^{+1.0}_{-0.77}$ & 	$-2.98^{+0.82}_{-0.59}$ & 	$-45.16^{+0.84}_{-0.66}$ & 	$-24.28^{+1.0}_{-0.72}$ & 	\textbf{0} & 	$-19.50^{+0.88}_{-0.69}$ & 	$-9.9^{+1.4}_{-1.4}$ \\


\hline
\hline
\end{tabular}
%\tablefoot{}
\end{center}
\label{tab:odd}
\end{table*}%




==> Table_Odds_IncludingPriors_Old.tex <==
\begin{table*}[]
\setlength{\extrarowheight}{3pt}
\caption{Natural logarithm of the Odd values ($\ln{Odd}=\ln{E}+\ln{P}$) for each model tested with repespect to the best model ($\ln{Odd} = 0$, in bold face).}
\small
\begin{center}
\begin{tabular}{l|ccc|ccc|ccc}
\hline
\hline
System & \multicolumn{9}{c}{$Ln{(Odd)}-Ln{(Odd_{\rm min})}$}   \\

     & {$\mathcal{F}$}1a & {$\mathcal{F}$}1b & {$\mathcal{F}$}1c & {$\mathcal{F}$}2a & {$\mathcal{F}$}2b & {$\mathcal{F}$}2c & {$\mathcal{F}$}3a & {$\mathcal{F}$}3b & {$\mathcal{F}$}3c   \\
\hline

corot-1b             &        \textbf{0} &        -19.21 &        -37.88 &        -41.62 &        -27.70 &        -45.96 &        -41.44 &        -28.11 &        -47.77 \\    
corot-2b             &      -11.37 &          \textbf{0} &        -18.15 &        -19.82 &         -8.55 &        -25.69 &        -20.07 &         -8.90 &        -26.95 \\    
corot-15b            &       -7.99 &          \textbf{0} &        -17.32 &        -19.33 &        -11.00 &        -28.44 &        -19.67 &        -11.75 &        -28.95 \\    
corot-18b            &       -6.11 &          \textbf{0} &        -15.07 &        -15.01 &         -8.35 &        -24.46 &        -15.13 &         -9.08 &        -24.28 \\    
epic211089792b       &       -2.82 &         -2.34 &         -5.20 &          \textbf{0} &         -8.21 &         -8.89 &        -10.50 &        -12.71 &        -11.95 \\    
gj3470b              &        \textbf{0} &        -12.26 &         -9.76 &         -3.71 &        -15.34 &        -13.40 &         -7.79 &        -20.11 &        -17.78 \\    
hat-p-12b            &        \textbf{0} &         -3.73 &         -1.28 &         -7.65 &         -8.08 &         -6.74 &         -3.22 &        -11.81 &        -10.28 \\    
hat-p-20b            &      -93.57 &          \textbf{0} &         -3.95 &       -106.06 &         -9.71 &        -13.18 &       -101.10 &         -9.06 &        -12.62 \\    
hat-p-23b            &      -12.09 &          \textbf{0} &        -17.61 &        -20.04 &         -8.85 &        -22.45 &        -20.67 &        -11.13 &        -21.96 \\    
hat-p-36b            &        \textbf{0} &         -1.22 &         -1.82 &         -8.03 &         -9.59 &        -10.58 &         -7.32 &        -12.54 &        -12.91 \\    
hat-p-54b            &        \textbf{0} &         -7.06 &         -9.17 &         -7.79 &        -15.37 &        -18.62 &         -7.84 &        -15.71 &        -20.34 \\    
hats-2b              &        \textbf{0} &        -12.16 &         -9.62 &         -8.62 &        -22.87 &        -19.14 &         -9.66 &        -22.59 &        -19.23 \\    
hats-9b              &        \textbf{0} &         -8.32 &        -11.36 &         -8.90 &        -17.49 &        -19.41 &         -8.55 &        -17.04 &        -18.42 \\    
k2-30b               &        \textbf{0} &         -9.22 &         -8.98 &         -7.47 &        -17.35 &        -17.28 &         -7.75 &        -17.51 &        -17.57 \\    
kepler-10b           &        \textbf{0} &        -59.03 &        -58.21 &        -54.59 &        -71.16 &        -65.18 &        -57.71 &        -66.47 &        -65.91 \\    
kepler-17b           &        \textbf{0} &         -3.27 &         -8.91 &         -8.13 &        -11.73 &        -17.43 &         -8.14 &        -11.70 &        -18.03 \\    
ogle-tr-113b         &        \textbf{0} &         -4.88 &         -2.51 &         -2.16 &        -15.51 &        -12.30 &         -1.49 &        -14.76 &        -11.64 \\    
ogle-tr-56b          &       -2.53 &          \textbf{0} &        -13.76 &        -12.77 &        -10.54 &        -23.79 &        -12.02 &         -9.22 &        -23.41 \\    
qatar-1b             &        \textbf{0} &        -11.26 &        -10.34 &         -9.03 &        -22.76 &        -19.81 &         -8.82 &        -21.43 &        -19.09 \\    
qatar-2b             &       -0.49 &         -2.89 &          \textbf{0} &         -8.93 &         -9.37 &         -6.07 &         -8.92 &        -12.47 &         -8.61 \\    
tres-3b              &       -4.41 &          \textbf{0} &        -24.56 &        -30.17 &        -35.93 &       -235.56 &        -17.09 &       -708.31 &       -156.54 \\    
tres-5b              &        \textbf{0} &        -15.18 &         -5.13 &         -9.19 &        -98.15 &        -25.88 &        -13.81 &        -83.85 &        -66.21 \\    
wasp-103b            &        \textbf{0} &        -14.91 &         -9.97 &         -9.12 &        -41.56 &        -19.63 &         -9.27 &        -62.35 &        -19.49 \\    
wasp-104b            &        \textbf{0} &         -6.81 &         -8.63 &         -7.61 &        -14.80 &        -16.57 &         -7.51 &        -14.93 &        -16.77 \\    
wasp-10b             &      -40.12 &          \textbf{0} &        -19.54 &        -24.73 &         -7.97 &        -29.00 &        -48.06 &         -7.95 &        -28.99 \\    
wasp-12b             &      -16.01 &          \textbf{0} &        -15.71 &        -24.57 &         -8.01 &        -23.72 &        -17.79 &         -6.97 &        -24.41 \\    
wasp-135b            &        \textbf{0} &         -6.01 &         -2.58 &         -7.86 &        -14.05 &        -10.71 &         -8.48 &        -16.90 &        -11.22 \\    
wasp-13b             &        \textbf{0} &        -10.85 &         -8.69 &         -7.73 &        -19.28 &        -18.00 &         -7.15 &        -19.54 &        -17.77 \\    
wasp-18b             &     -134.35 &          \textbf{0} &        -17.42 &       -143.02 &         -8.75 &        -26.04 &       -142.99 &         -8.66 &        -26.37 \\    
wasp-19b             &       -8.94 &          \textbf{0} &        -14.51 &        -16.85 &         -8.44 &        -22.65 &        -16.86 &         -6.93 &        -23.06 \\    
wasp-23b             &        \textbf{0} &         -5.10 &         -7.80 &         -7.25 &        -12.97 &        -15.55 &         -7.57 &        -12.90 &        -15.64 \\    
wasp-2b              &      -10.01 &          \textbf{0} &        -17.45 &        -17.16 &         -7.00 &        -25.23 &        -17.48 &         -7.66 &        -25.13 \\    
wasp-35b             &        \textbf{0} &        -12.29 &         -9.32 &         -7.69 &        -20.33 &        -17.56 &         -7.63 &        -20.68 &        -17.32 \\    
wasp-36b             &      -14.83 &          \textbf{0} &        -12.75 &        -11.19 &         -8.96 &        -20.94 &        -11.48 &         -9.62 &        -21.46 \\    
wasp-42b             &      -12.44 &          \textbf{0} &         -2.98 &         -7.85 &         -7.88 &        -11.26 &        -20.11 &         -7.95 &        -10.53 \\    
wasp-43b             &      -21.17 &          \textbf{0} &        -12.60 &        -11.78 &         -8.40 &        -21.44 &        -11.90 &         -8.23 &        -21.42 \\    
wasp-46b             &       -5.31 &          \textbf{0} &        -15.14 &        -14.07 &         -9.38 &        -24.11 &        -14.15 &         -8.83 &        -23.97 \\    
wasp-49b             &        \textbf{0} &        -12.69 &         -9.41 &         -7.24 &        -21.43 &        -17.39 &         -7.46 &        -20.85 &        -17.77 \\    
wasp-4b              &       -6.01 &          \textbf{0} &        -13.62 &        -11.96 &         -9.06 &        -20.77 &        -13.71 &         -7.93 &        -21.60 \\    
wasp-50b             &        \textbf{0} &         -5.69 &         -8.63 &         -7.77 &        -13.89 &        -16.70 &         -7.11 &        -14.00 &        -16.43 \\    
wasp-52b             &        \textbf{0} &        -11.11 &         -8.42 &         -7.70 &        -18.82 &        -16.30 &         -7.24 &        -19.01 &        -16.04 \\    
wasp-5b              &      -16.18 &         -9.44 &        -24.26 &        -11.75 &          \textbf{0} &         -9.84 &        -24.33 &        -17.74 &        -32.30 \\    
wasp-65b             &        \textbf{0} &        -13.26 &         -9.31 &         -8.18 &        -21.64 &        -17.70 &         -8.26 &        -21.70 &        -17.90 \\    
wasp-68b             &        \textbf{0} &         -6.76 &         -3.57 &         -8.04 &        -14.74 &        -11.73 &         -0.16 &        -13.12 &         -9.22 \\    
wasp-77ab            &        \textbf{0} &        -10.29 &         -4.87 &         -5.51 &        -16.91 &        -12.54 &         -7.65 &        -17.42 &        -12.66 \\    
wasp-80b             &        \textbf{0} &         -6.75 &        -16.65 &        -15.52 &        -18.94 &        -24.20 &        -10.12 &        -19.98 &        -23.17 \\    
wasp-98b             &        \textbf{0} &        -13.70 &         -9.95 &         -8.57 &        -23.05 &        -19.68 &         -8.24 &        -23.68 &        -19.97 \\    
wts-2b               &        \textbf{0} &        -12.37 &        -10.81 &        -10.22 &        -25.34 &        -21.38 &         -8.94 &        -23.25 &        -19.43 \\    





\hline
\hline
\end{tabular}
%\tablefoot{}
\end{center}
\label{tab:odd}
\end{table*}%




==> Table_priors.tex <==
\begin{table*}[]
\setlength{\extrarowheight}{7pt}
\caption{Priors for the different models tested.}
\begin{center}
\begin{tabular}{lccccccccc}
\hline
\hline
 &  &  &  & \multicolumn{2}{c}{(i)} & \multicolumn{2}{c}{(ii)} & \multicolumn{2}{c}{(iii)}  \\
Model ID & $V_{\rm sys}$ & $K_p$ & $K_t$ & $e\cos{\omega}$ & $e\sin{\omega}$  \\
\hline
\multicolumn{6}{l}{\it No trojan}\\ \hline
$\mathcal{F}$1a & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & 0  & $e=0$  & $\omega=\pi/2$ & $e=0$  & $\omega=\pi/2$ & $e=0$  & $\omega=\pi/2$  \\
$\mathcal{F}$1b & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & 0  &  &  \\
$\mathcal{F}$1c & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & 0  &  &  \\ \hline
\multicolumn{6}{l}{\it Trojan at $L_4$ }\\ \hline
$\mathcal{F}$2a & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & $\mathcal{M}(K_a;K_{\rm max})$  &  &  \\
$\mathcal{F}$2b & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & $\mathcal{M}(K_a;K_{\rm max})$  &  &  \\
$\mathcal{F}$2c & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & $\mathcal{M}(K_a;K_{\rm max})$  &  &  \\ \hline
\multicolumn{6}{l}{\it Trojan at $L_5$}\\ \hline
$\mathcal{F}$3a & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & $\mathcal{M}(K_a;K_{\rm max})$  &  &  \\
$\mathcal{F}$3b & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & $\mathcal{M}(K_a;K_{\rm max})$  &  &  \\
$\mathcal{F}$3c & $\mathcal{U}(a;b)$ & $\mathcal{M}(K_a;K_{\rm max})$ & $\mathcal{M}(K_a;K_{\rm max})$  &  &  \\

\hline
\hline
\end{tabular}
\tablefoot{$\mathcal{N}(\mu;\sigma^{2})$ is a normal distribution with mean $\mu$ and width $\sigma^{2}$, $\mathcal{U}(a;b)$ is a uniform distribution between $a$ and $b$, $\mathcal{S}(a;b)$ is a sine distribution between $a$ and $b$, $\beta(a;b)$ is a Beta distribution with parameters $a$ and $b$, and $\mathcal{P}(n;a;b)$ is a power-law distribution of exponent $n$ between $a$ and $b$.}
\tablebib{The choice of prior for the orbital eccentricity is described in \citet{kipping13}.}
\end{center}
\label{tab:priors}
\end{table*}%



%\multicolumn{3}{l}{\it Orbital parameters}\\
%&&\\
%Orbital period $P$ [d] & $\mathcal{N}(4.09803;1\times10^{-3})$ & $\mathcal{N}(2.996;1\times10^{-3})$\\
%Epoch of first transit T$_{0}$ [BJD$_{\rm TDB}$] - 2450000 & $\mathcal{N}(7063.826;0.1)$ & $\mathcal{N}(7141.35;0.1)$\\
%Orbital eccentricity $e$ & $\beta(0.867;3.03)$ & 0 (fixed) \\
%Argument of periastron $\omega$ [\degr] & $\mathcal{U}(0;360)$ & -- \\
%Inclination $i$ [\degr] & $\mathcal{S}(70;90)$ & $\mathcal{S}(70;90)$\\
%&&\\
%\hline
%\multicolumn{3}{l}{\it Planetary parameters}\\
%&&\\
%Radial velocity amplitude $K$ [m/s] & $\mathcal{U}(0;1000)$ & $\mathcal{U}(0;1000)$\\
%Planet-to-star radius ratio $a/R_{\star}$ & $\mathcal{U}(0; 0.5)$ & $\mathcal{U}(0; 0.5)$\\
%&&\\
%\hline
%\multicolumn{3}{l}{\it Stellar parameters}\\
%&&\\
%Effective temperature $T_{\rm eff}$ [K] & $\mathcal{N}(5573;38)$ & $\mathcal{N}(6139;50)$ \\
%Surface gravity $\log{g}$ [g/cm$^{2}$] & $\mathcal{N}(4.32;0.20)$ & $\mathcal{N}(4.07;0.21)$\\
%Iron abundance [Fe/H] [dex] & $\mathcal{N}(0.14;0.03)$ & $\mathcal{N}(0.11;0.04)$\\
%Reddening E(B-V) [mag] & $\mathcal{U}(0;1)$ & $\mathcal{U}(0;1)$\\
%Systemic radial velocity V$_{\rm sys}$ [km/s] & $\mathcal{U}(-100, 100)$ & $\mathcal{U}(-100, 100)$\\
%Distance to Earth $d$ [pc] & $\mathcal{P}(2;10;1000)$ & $\mathcal{P}(2;10;1000)$\\
%Linear limb darkening coefficient ua & $\mathcal{U}(0, 1.2)$ & $\mathcal{U}(0, 1.2)$\\
%Quadratic limb darkening coefficient ub & $\mathcal{U}(0, 1.2)$ & $\mathcal{U}(0, 1.2)$\\
%&&\\
%\hline
%\multicolumn{3}{l}{\it Instrumental parameters}\\
%&&\\
%CAFE radial velocity jitter $\sigma_{\rm RV,CAFE}$ [m/s] & -- & $\mathcal{U}(0;100)$ \\
%SOPHIE radial velocity jitter $\sigma_{\rm RV,SOPHIE}$ [m/s] & $\mathcal{U}(0;100)$ & $\mathcal{U}(0;100)$\\
%HARPS-N radial velocity jitter $\sigma_{\rm RV,HARPS-N}$ [m/s] & $\mathcal{U}(0;100)$ & $\mathcal{U}(0;100)$\\
%CAFE -- SOPHIE radial velocity offset $\Delta$ RV$_{S,CAFE}$ [m/s] & $\mathcal{U}(-1000;1000)$ & $\mathcal{U}(-1000;1000)$\\
%HARPS-N -- SOPHIE radial velocity offset $\Delta$ RV$_{S,H-N}$  [m/s] & $\mathcal{U}(-1000;1000)$ & $\mathcal{U}(-1000;1000)$\\
%SED jitter $\sigma_{\rm SED}$ [mag] & $\mathcal{U}(0;1)$ & $\mathcal{U}(0;1)$\\
%\hline
%\hline
%\end{tabular}
%\tablefoot{$\mathcal{N}(\mu;\sigma^{2})$ is a normal distribution with mean $\mu$ and width $\sigma^{2}$, $\mathcal{U}(a;b)$ is a uniform distribution between $a$ and $b$, $\mathcal{S}(a;b)$ is a sine distribution between $a$ and $b$, $\beta(a;b)$ is a Beta distribution with parameters $a$ and $b$, and $\mathcal{P}(n;a;b)$ is a power-law distribution of exponent $n$ between $a$ and $b$.}
%\tablebib{The choice of prior for the orbital eccentricity is described in \citet{kipping13}.}
%\end{center}
%\label{tab:priors}
%\end{table*}%


